Feel the Tension: Manipulation of Deformable Linear Objects in Environments with Fixtures using Force Information

Humans are able to manipulate Deformable Linear Objects (DLOs) such as cables and wires, with little or no visual information, relying mostly on force sensing. In this work, we propose a reduced DLO model which enables such blind manipulation by keeping the object under tension. Further, an online model estimation procedure is also proposed. A set of elementary sliding and clipping manipulation primitives are defined based on our model. The combination of these primitives allows for more complex motions such as winding of a DLO. The model estimation and manipulation primitives are tested individually but also together in a real-world cable harness production task, using a dual-arm YuMi, thus demonstrating that force-based perception can be sufficient even for such a complex scenario.

==> preliminaries.tex <==
Before introducing the proposed DLO model and manipulation primitives, we present the notation used in the following sections as well as conventions used to describe the dual-arm robotic setup.

Let $\{h_a\}$ and $\{h_b\}$ denote two coordinate frames. Frame $\{h_b\}$ can be represented with respect to $\{h_b\}$ through a translation $\prescript{a}{}{\mathbf{p}_b} \in \mathbb{R}^3$ and a rotation $\prescript{a}{b}{\mathbf{R}}\in SO(3)$. Therefore, the subscript $b$ indicates the transformed frame and the relative to the superscript $a$ indicates the reference frame. Note that $SO(3)$ refers to the Lie group for 3D rotations. Bold letters are used to define vectors or matrices and underlined vectors indicate normalisation, $\textbf{\underline{x}} = \frac{\textbf{x}}{\|\textbf{x}\|}$. The identity matrix is denoted by $\mathbf{I}_n \in\mathbb{R}^{n\times n}$, while the zero matrix includes both dimensions in the subscript, as $\mathbf{0}_{n\times m}$. Finally, the dot product between vectors $\mathbf{a}$ and $\mathbf{b}$ is denoted by $\mathbf{a} \cdot \mathbf{b} = c$, while the cross product is denoted by $ \mathbf{a} \times \mathbf{b} = \mathbf{c}$.

The robotic setup can be seen in Fig. \ref{fig:YuMi_frames}, where $\{h_{FT}\}$ is the FT sensing frame, $\{h_{l}\}$ the frame associated to the tool tip at the left gripper, and $\{h_{r}\}$ at the right gripper. A fixture frame is denoted as $\{h_{fix}\}$ and the world frame as $\{h_{world}\}$. 
